A Calculus for Amortized Expected Runtimes

We develop a weakest-precondition-style calculus \`a la Dijkstra for reasoning about amortized expected runtimes of randomized algorithms with access to dynamic memory - the $\textsf{aert}$ calculus. Our calculus is truly quantitative, i.e. instead of Boolean valued predicates, it manipulates real-valued functions. En route to the $\textsf{aert}$ calculus, we study the $\textsf{ert}$ calculus for reasoning about expected runtimes of Kaminski et al. [2018] extended by capabilities for handling dynamic memory, thus enabling compositional and local reasoning about randomized data structures. This extension employs runtime separation logic, which has been foreshadowed by Matheja [2020] and then implemented in Isabelle/HOL by Haslbeck [2021]. In addition to Haslbeck's results, we further prove soundness of the so-extended $\textsf{ert}$ calculus with respect to an operational Markov decision process model featuring countably-branching nondeterminism, provide intuitive explanations, and provide proof rules enabling separation logic-style verification for upper bounds on expected runtimes. Finally, we build the so-called potential method for amortized analysis into the $\textsf{ert}$ calculus, thus obtaining the $\textsf{aert}$ calculus. Since one needs to be able to handle changes in potential which can be negative, the $\textsf{aert}$ calculus needs to be capable of handling signed random variables. A particularly pleasing feature of our solution is that, unlike e.g. Kozen [1985], we obtain a loop rule for our signed random variables, and furthermore, unlike e.g. Kaminski and Katoen [2017], the $\textsf{aert}$ calculus makes do without the need for involved technical machinery keeping track of the integrability of the random variables. Finally, we present case studies, including a formal analysis of a randomized delete-insert-find-any set data structure [Brodal et al. 1996].

==> dynamic_list_ert_proof.tex <==
%\begin{figure}
%	
%	\begin{align*}
%		&\geqannotate{\pureemp{\aoff<\asize} \sepadd \earray{\ahead}{\asize} \sepadd \emprun{1} \sepadd (\pureemp{\aoff+1 \neq \asize} \rtmin \emprun{\asize})} \\
%		%
%		&\ertannotate{\pureemp{\aoff + 1 =\asize} \sepadd \emprun{1}\sepadd \emprun{\asize}  \sepadd \earray{\ahead}{s} \sepadd \pureemp{\aoff  + 1 < 2\cdot \asize }} \\
%		%
%		 &\phantannotate{\quad \rrtmin \pureemp{\aoff + 1 \neq \asize} \sepadd \emprun{1}\sepadd \earray{\ahead}{\asize} \sepadd \pureemp{\aoff  + 1 <\asize}} \\
%		%
%		&\IF{\aoff + 1 = \asize} \\
%		%
%		&\qquad \frameannotate{\emprun{1}\sepadd \emprun{\asize}  \sepadd \earray{\ahead}{s} \sepadd \pureemp{\aoff  + 1 < 2\cdot \asize }}{} \\
%		%
%		& \qquad  \ALLOC{\ahead'}{2\cdot\asize } \fatsemi \\
%		%
%		&\qquad \geqannotate{\emprun{1}\sepadd \emprun{\asize}  \sepadd \earray{\ahead}{s} \sepadd \earray{\ahead'}{2\cdot \asize } \sepadd \pureemp{\aoff  + 1 < 2\cdot \asize }}{} \\
%		%
%		&\qquad \frameannotate{\emprun{1}\sepadd \emprun{\asize} \sepadd \pureemp{2\cdot\asize  \geq s} \sepadd \earray{\ahead}{s} \sepadd \earray{\ahead'}{2\cdot \asize } \sepadd \pureemp{\aoff  + 1 < 2\cdot \asize }}{} \\
%		%
%		& \qquad \arraycopy{\ahead}{\asize}{\ahead'} \fatsemi \\
%		%
%		&\qquad \frameannotate{\emprun{1}\sepadd \earray{\ahead}{s} \sepadd \earray{\ahead'}{2\cdot \asize } \sepadd \pureemp{\aoff  + 1 < 2\cdot \asize }}{} \\
%		%
%		&\qquad \arraydelete{\ahead}{\asize} \fatsemi \\
%		%
%		& \qquad \ertannotate{\emprun{1}\sepadd \earray{\ahead'}{2\cdot \asize } \sepadd \pureemp{\aoff  + 1 < 2\cdot \asize }} \\
%		%
%		& \qquad \ASSIGN{\ahead}{\ahead'}\fatsemi \\
%		%
%		& \qquad \ertannotate{\emprun{1}\sepadd \earray{\ahead}{2\cdot \asize } \sepadd \pureemp{\aoff  + 1 < 2\cdot \asize }} \\
%		%
%		& \qquad \ASSIGN{\asize}{2\cdot \asize }\\
%		%
%		& \qquad \annotate{\emprun{1}\sepadd \earray{\ahead}{\asize} \sepadd \pureemp{\aoff  + 1 <\asize}} \\
%		%
%		& \} \\
%		%
%		& \geqannotate{\emprun{1}\sepadd \earray{\ahead}{\asize} \sepadd \pureemp{\aoff  + 1 <\asize}} \\
%		%
%		& \ertannotate{\emprun{1}\sepadd \validpointer{\ahead + \aoff + 1} \sepadd 0} \\
%		%
%		&\ASSIGN{\aoff}{\aoff +1}\fatsemi \\
%		%
%		&\framemutannotate{\emprun{1}\sepadd \validpointer{\ahead + \aoff} \sepadd 0} \\
%		%
%		& \HASSIGN{\ahead + \aoff}{y}\fatsemi \\
%		%
%		&\geqannotate{\emprun{1}\sepadd \singleton{\ahead + \aoff}{y} \sepadd 0} \\
%		%
%		&\ertannotate{\emprun{1}\sepadd 0} \\
%		%
%		& \TICK{1} \\
%		%
%		& \annotate{0} \\
%	\end{align*}
%	
%	\caption{Dynamic List Runtime Verification. TODO: Use nice boxes for frames}
%	\label{fig:dynamic_list_ert_proof}
%\end{figure}





\begin{figure}
	
	\begin{align*}
	&\geqannotate{\pureemp{\aoff\leq \asize \wedge \asize \geq 1} \sepadd \earray{\ahead}{\asize} \sepadd \emprun{1} \sepadd (\iverson{\aoff = \asize} \cdot \emprun{\asize})} \\
	%
	&\ertannotate{\iverson{\aoff  =\asize} \cdot (\emprun{1} \sepadd \pureemp{\aoff \leq \asize \wedge \asize \geq 1} \sepadd  \emprun{\asize} \sepadd \earray{\ahead}{\asize})
	+ \iverson{\aoff  \neq \asize} \cdot (\emprun{1} \sepadd 0 \sepadd \ivalidpointer{\ahead + \aoff} )} \\
	%
	&\IF{\aoff  = \asize} \\
	%
	&\qquad \unframeannotate{\emprun{1} \sepadd \pureemp{\aoff \leq \asize \wedge \asize \geq 1} \sepadd  \emprun{\asize} \sepadd \earray{\ahead}{\asize} }{} \\
	%
	&\qquad \annotate{\iemp} \\
	%
	& \qquad  \ALLOC{\ahead'}{2\cdot\asize } \fatsemi \\
	%
	&\qquad \frameannotate{\earray{\ahead'}{2\cdot \asize }}{} \\
	%
    &\qquad \geqannotate{\emprun{1} \sepadd \pureemp{\aoff \leq \asize \wedge \asize \geq 1} \sepadd  \emprun{\asize} \sepadd \earray{\ahead}{\asize} \sepadd \earray{\ahead'}{2\cdot \asize }}{} \\
	%
	&\qquad \unframeannotate{\emprun{1} \sepadd \pureemp{\aoff \leq \asize \wedge \asize \geq 1} \sepadd \pureemp{2\cdot \asize \geq \asize } \sepadd \emprun{\asize} \sepadd \earray{\ahead}{\asize} \sepadd \earray{\ahead'}{2\cdot \asize }}{} \\
	%
	&\qquad \annotate{\pureemp{2\cdot \asize \geq \asize } \sepadd \emprun{\asize} \sepadd \earray{\ahead}{\asize} \sepadd \earray{\ahead'}{2\cdot \asize }} \\
	%
	& \qquad \arraycopy{\ahead}{\asize}{\ahead'} \fatsemi \\
	%
	&\qquad \frameannotate{\earray{\ahead}{\asize} \sepadd \earray{\ahead'}{2\cdot \asize}}{} \\
	%
	&\qquad \geqannotate{\emprun{1} \sepadd \pureemp{\aoff \leq \asize \wedge \asize \geq 1} \sepadd \earray{\ahead}{\asize} \sepadd \earray{\ahead'}{2\cdot \asize} }{} \\
	%
	&\qquad \unframeannotate{\emprun{1} \sepadd 0 \sepadd \ivalidpointer{\ahead' + \aoff}  \sepadd \earray{\ahead}{\asize}}{} \\
	%
	&\qquad \annotate{\earray{\ahead}{\asize}} \\
	%
	&\qquad \arraydelete{\ahead}{\asize} \fatsemi \\
	%
	& \qquad \frameannotate{\iemp }{} \\
	%
	& \qquad \ertannotate{\emprun{1} \sepadd 0 \sepadd \ivalidpointer{\ahead' + \aoff} } \\
	%
	& \qquad \ASSIGN{\ahead}{\ahead'}\fatsemi \\
	%
	& \qquad \ertannotate{\emprun{1} \sepadd 0 \sepadd \ivalidpointer{\ahead + \aoff} } \\
	%
	& \qquad \ASSIGN{\asize}{2\cdot \asize }\\
	%
	& \qquad \annotate{\emprun{1} \sepadd 0 \sepadd \ivalidpointer{\ahead + \aoff} } \\
	%
	& \} \\
	%
	%
	%
	&\unframeannotate{\emprun{1} \sepadd 0 \sepadd \ivalidpointer{\ahead + \aoff} }{} \\
	%
	&\mutannotate{\ivalidpointer{\ahead + \aoff}} \\
	%
	& \HASSIGN{\ahead + \aoff}{y}\fatsemi \\
	%
	&\frameannotate{\isingleton{\ahead + \aoff}{y}}{} \\
	%
	&\geqannotate{\emprun{1} \sepadd 0 \sepadd \isingleton{\ahead + \aoff}{y}} \\
	%
	&\ertannotate{\emprun{1}\sepadd 0} \\
	%
	&\ASSIGN{\aoff}{\aoff +1}\fatsemi \\
	%
	&\ertannotate{\emprun{1}\sepadd 0} \\
	%
	& \TICK{1} \\
	%
	& \annotate{0} \\
	\end{align*}
	
	\caption{Dynamic List Runtime Verification.}
	\label{fig:dynamic_list_ert_proof}
\end{figure}

==> rsl.tex <==
\subsection*{Separating Connectives between Runtimes}


%
%As an example consider a quantity $f$ that counts the number of pointers to $\nil$ in the heap, i.e. $f(s,h) = |\{ v \in \dom{h} ~|~ h(v) = \nil \}|$.
%The expectation $\singleton{x}{\nil} \sepcon f$ then intuitively removes a pointer to $\nil$ originating from address $s(x)$ from the heap and afterwards measures the remaining number of pointers to $\nil$.
%In particular, the whole expectation is set to $0$ if $s(x)$ does not point to $0$.
%The separating conjunction thus acts to carve out a fragment from the heap before taking a quantitative measurement.



%


==> soundness.tex <==
%\section{Soundness}\label{s:op}
%
%We show that RSL is sound with respect to a small-step operational semantics based on Markov decision processes (MDPs)---a widely used probabilistic model.
%We first define individual execution steps, then recapitulate the essentials of MDPs, and finally discuss how the expected reward collected by the MDP induced by our operational semantics coincides with the RSL calculus.
%
%
%\subsection{Execution steps}
%
%\paragraph{Configurations}
%The set of \emph{program configurations} is given by
%\[
%  \Confs \qeq 
%  \hpgcl ~\times~ \Stacks ~\times~ \Heaps 
%  \quad\cup\quad
%  \{\term, \fail\} ~\times~ \Stacks ~\times~ \Heaps 
%  \quad\cup\quad
%   \{\sink\}~.
%\]
%A configuration
%is an \hpgcl program $C$ together, an identifier $\term$ indicating successful (\ie, without memory errors) termination, or $\fail$, which indicates that the program encountered a memory error, together with a program state $(\sk,\hh)$. For technical reasons, we also added a $\sink$ state in which we stay forever after program termination.
%
%\paragraph{Execution relation}
%The steps of our operational semantics are given by an execution relation
%\[
%  \mstep{}{}~ \quad\subseteq\quad \Confs ~\times~ \textsf{Prob} ~\times~ \textsf{Choice} ~\times~ \Confs~,
%\]
%where $\textsf{Prob}$ is the set of transition probabilities\footnote{Formally, we set $\textsf{Prob} = ([0,1] \cap \Rats) \cup \{1-\sfrac{1}{2}\}$, where the fake value $1-\sfrac{1}{2}$ allows representing two distinct steps from the same configuration to the same configuration with probability $\sfrac{1}{2}$.} and $\textsf{Choice} = \Nats$ is used to indicate nondeterministic choices, \eg, the address chosen during memory allocation.
%Hence, a step $c \mstep{p}{u} c'$ (our notation for $(c, p, u, c') \in\, \mstep{}{}$) indicates an execution \emph{step} from configuration $c$ to configuration $c'$ with probability $p$ and nondeterministic choice $u$.
%To avoid notational clutter, we often omit the transition probability $p$ if $p=1$ and
% the choice $n$ if if no choice is needed and we default to $n = 0$.
%Formally, the execution relation $\mstep{}{}$ is given by the inference rules in \Cref{fig:op:rules}.
%Most of the rules are standard for heap-manipulating and probabilistic programs (cf.,~\cite{todo}).
%\cmin{TODO}
%Notice that our execution relation is never stuck, \ie for every configuration $c$ there exist $p \in \textsf{Prob}$, $\ma \in \textsf{Choice}$ and $c' \in \Confs$ such that $c \mstep{p}{\ma} c'$.
%
%For every choice $n \in \textsf{Choice}$ and every configuration $c \in Confs$, our execution relation $\mstep{}{}$ induces a probability distribution over successor configurations. Formally, let $\MPOP(c,u,c')$ be the accumulated probability of moving from $c$ to some fixed configuration $c'$ using choice $n$, \ie, 
%\begin{align}
%    \MPOP\colon \Confs \times \textsf{Choices} \times \Confs,
%    \qquad
%    (c,\ma,c') \mapsto \sum_{p\colon c ~\mstep{p}{\ma}~ c'} p~.
%    \label{eq:mpop}
%\end{align}
%Then, by construction, for all $c \in \Confs$ and all $n \in \textsf{Choice}$, we have $\sum_{c' \in \Confs} \MPOP(c,u,c') = 1$.
%
%\begin{figure}[t]
%\small
%\begin{align*}
%& \conf{\TICK{e}}{\sk}{\hh} \qmstep{}{} \tconf{\sk}{\hh}
%  \hspace{3em}
%  \tconf{\sk}{\hh} \qmstep{}{} \sink 
%  \hspace{3em} 
%  \sink \mstep{}{} \sink
%  \hspace{3em} 
%  \conf{\fail}{\sk}{\hh} \mstep{}{} \sink
%\\
%& \conf{\PCHOICE{C_1}{p}{C_2}}{\sk}{\hh} \qmstep{p}{} \conf{C_1}{\sk}{\hh}
%  \hspace{5em}
%  \conf{\PCHOICE{C_1}{p}{C_2}}{\sk}{\hh} \qmstep{1-p}{} \conf{C_2}{\sk}{\hh}
%\\
%& \conf{\ASSIGN{x}{e}}{\sk}{\hh} \qmstep{}{} \tconf{\sk\subst{x}{\sk(e)}}{\hh}
%  \hspace{3em}
%  \conf{\ITE{\varphi}{C_1}{C_2}}{\sk}{\hh} \qmstep{}{} 
%  \begin{cases}
%    \conf{C_1}{\sk}{\hh} & \tif \sk \models \varphi \\
%    \conf{C_2}{\sk}{\hh} & \tif \sk \not\models \varphi
%  \end{cases}
%\\
%& \conf{\ALLOC{x}{e}}{\sk}{\hh} \qmstep{}{u} 
%  \tconf{\sk\subst{x}{u}}{\hh \sepcon \{\, u \mapsto \underbrace{0,\ldots,0}_{\text{$n$ times}}\,\}}, \qif n = \sk(e),\quad u,\ldots,u+n-1 \notin \dom{\hh}
%\\
%& \conf{\ASSIGNH{x}{e}}{\sk}{\hh} \qmstep{}{}
%  \begin{cases}
%    \tconf{\sk\subst{x}{\hh(v)}}{\hh} & \qif \sk(e) = v \in \dom{\hh} \\
%    \conf{\fail}{\sk}{\hh} & \qif \sk(e) \notin \dom{\hh}
%  \end{cases}
%\\
%& \conf{\HASSIGN{e}{e'}}{\sk}{\hh} \qmstep{}{}
%  \begin{cases}
%    \tconf{\sk}{\hh\subst{v}{\sk(e')}} & \qif \sk(e) = v \in \dom{\hh} \\
%    \conf{\fail}{\sk}{\hh} & \qif \sk(e) \notin \dom{\hh}
%  \end{cases}
%\\
%& \conf{\FREE{e}}{\sk}{\hh} \qmstep{}{}
%  \begin{cases}
%    \tconf{\sk}{\hh'} & \qif \hh = \hh' \sepcon \{ \sk(e) \mapsto v \} ~\text{for some}~v \in \Vals \\
%    \conf{\fail}{\sk}{\hh} & \quad\text{otherwise}
%  \end{cases}
%\\
%& \conf{\WHILEDO{\varphi}{C}}{\sk}{\hh} \qmstep{}{} 
%  \begin{cases}
%    \conf{\COMPOSE{C}{\WHILEDO{\varphi}{C}}}{\sk}{\hh} & \qif \sk \models \varphi \\
%    \conf{\term}{\sk}{\hh} & \qif \sk \not\models \varphi
%  \end{cases}
%\\
%&
%  \inference{
%    \conf{C_1}{\sk}{\hh}
%    \qmstep{p}{u}
%    \conf{C_1'}{\sk'}{\hh'}
%  }{
%    \conf{\COMPOSE{C_1}{C_2}}{\sk}{\hh}
%    \qmstep{p}{u}
%    \conf{\COMPOSE{C_1'}{C_2}}{\sk'}{\hh'}
%  }
%  %
%  \hspace{1em}
%  %
%  \inference{
%    \conf{C_1}{\sk}{\hh}
%    \qmstep{p}{u}
%    \tconf{\sk'}{\hh'}
%  }{
%    \conf{\COMPOSE{C_1}{C_2}}{\sk}{\hh}
%    \qmstep{p}{u}
%    \conf{C_2}{\sk'}{\hh'}
%  }
%  %
%  \hspace{1em}
%  %
%  \inference{
%    \conf{C_1}{\sk}{\hh}
%    \qmstep{p}{u}
%    \conf{\fail}{\sk}{\hh}
%  }{
%    \conf{\COMPOSE{C_1}{C_2}}{\sk}{\hh}
%    \qmstep{p}{u}
%    \conf{\fail}{\sk}{\hh}
%  }
%\end{align*}
%\caption{The inference rules determining the execution relation $\mstep{}{}$ of the operational semantics.}
%\label{fig:op:rules}
%\end{figure}
%
%
%\subsection{Markov Decision Processes}
%
%Our actual operational semantics is not just an execution relation but a Markov decision process. 
%We briefly summarize the underlying foundations; we broadly adhere to the notation in the textbook by~\citet[Chapter 10]{DBLP:books/daglib/0020348}.
%However, we consider Markov decision processes with infinitely many states, infinitely many actions, and (non-discounted) rewards. A thorough discussion of such MDPs is found in \cite[Chapter 7]{puterman2005markov}.
% 
%\begin{definition}[Markov Decision Process (MDP)]
%	A \emph{Markov decision process} $\MDP$ is a tuple 
%	\[ \MDP \eeq \left( \MS, \MA, \MP, \MI, \MR \right)~, \]
%	where 
%	$\MS$ is a countable set of \emph{states},
%	$\MA$ is a countable set of \emph{actions},
%	$\MP\colon \MS \times \MA \times \MS \to [0,1]$ is the \emph{transition probability function}\footnote{i.e., for all states $\ms \in \MS$ and actions $\ma \in \MA$, we have $\sum_{\ms' \in \MS} \MP(\ms,\ma,\ms') = 1$}, 
%	$\MI \in \MS$ is the \emph{initial state}, and 
%	$\MR\colon \MS \to \PosRealsInf$ assigns to every state a reward collected upon leaving a state. 
%\end{definition}
%
%Throughout this subsection, we fix an MDP $\MDP = \left( \MS, \MA, \MP, \MI, \MR \right)$ to reduce clutter.
%
%\begin{definition}[Scheduler]
%	A \emph{scheduler} of MDP $\MDP$ is a function $\msched\colon \MS^{+} \to \MA$
%	that chooses an action for every non-empty sequence of states. We denote by $\MSCHED$ the set of all schedulers.
%\end{definition}
%
%\begin{definition}[Finite $\msched$-paths]
%  Given a scheduler $\msched$, an $\msched$-\emph{path} $\mpath$ of length $n \in \Nats$
%  is a sequence of states $\mpath = \ms_0 \ldots \ms_{n-1}$ such that
%  (1) $\ms_0 = \MI$ and (2) for all $i \in \{1, \ldots, n-1\}$, we have $\MP(\ms_{i-1}, \msched(\ms_0 \ldots \ms_{i-1}), \ms_i) > 0$. 
%  We denote by $\mpaths{n}{\msched}$ the set of all $\msched$-paths of length $n$. 
%\end{definition}
%
%We lift the transition function $\MP$ and the reward function $\MR$ to $\msched$-paths $\mpath = \ms_0 \ldots \ms_{n-1}$:
%
%\begin{align*}
% \MP(\ms_0 \ldots \ms_{n-1}) \eeq \prod_{i=1}^{n-1} \MP(\ms_{i-1}, \msched(\ms_0 \ldots \ms_{i-1}), \ms_i)
% \qquad\qquad
% \MR(\ms_0 \ldots \ms_{n-1}) \eeq \sum_{i=0}^{n-1} \MR(\ms_{i})
%\end{align*}
%
%
%\begin{definition}[Total expected reward]
%  \begin{align*}
%  	\ExpRew{\MDP} \qeq 
%  	\sup_{\msched \in \MSCHED} ~ \sup_{n \in \Nats} ~\sum_{\mpath \in \mpaths{\MDP}{\msched}} \MP(\mpath) \cdot \MR(\mpath)
%  \end{align*}
%\end{definition}
%
%\subsection{The Operational Markov Decision Process}
%
%The \emph{operational MDP} $\MDPOP{C,f,\sk,\hh}$, which captures the semantics of an \hpgcl program $C$ 
%with respect to a runtime $\rta \in \T$ and an initial program state $(\sk,\hh) \in \Stacks \times \Heaps$, is defined as
%	\[ 
%	  \MDPOP{C,f,\sk,\hh} \qeq \left(\, \Confs,~ \textsf{Choice},~ \MPOP,~ (\conf{C}{\sk}{\hh}),~ \MROP \,\right)~, 
%	\]
%where the set of states consists of all program configurations, the set of actions consist of all choices, \ie $\MA = \textsf{Choice} = \Nats$, $\MPOP$ is the transition probability function induced by our execution relation defined in \Cref{fig:op:rules} (cf., \cref{eq:mpop}), and the reward function $\MROP$ is given by
%%
%\begin{align*}
%  \MROP\colon \Confs \to \PosRealsInf,
%  \qquad\qquad 
%  c \mapsto
%  \begin{cases}
%    \sk(e),        & \qif c = (\conf{\TICK{e}}{\sk}{\hh}) \\
%    \rta(\sk,\hh), & \qif c = (\conf{\term}{\sk}{\hh}) \\
%    \infty,        & \qif c = (\conf{\fail}{\sk}{\hh}) \\
%    0,             & \quad \text{otherwise}. 
%  \end{cases}
%\end{align*}
%%
%In other words, the reward models the cost represented by $\TICK{e}$ statements and
%the postruntime $\rta$ needed after termination. Morever, we take a demoninic view on nondeterminism and assume the program may have an unbounded runtime if a memory error occurs. Hence, the reward assigned to the error state $\fail$ is infinity. 
%%
%
%%
%With these notions in place, we can state the main result of this section: our runtime separation logic is sound in the sense that it characterizes exactly the expected reward of operational MDPs:

\subsection{Soundness}\label{s:op}

We show that RSL is sound with respect to the small-step operational semantics based on Markov decision processes introduced in \Cref{s:op-semantics}.

\begin{theorem}[Soundness]\label{thm:ert-sound-op}
  For all $\hpgcl$ programs $C$, runtimes $\rta \in \T$, and program states $(\sk,\hh)$,
  \begin{align*}
    \ert{C}{\rta}(\sk,\hh) \qeq 
    \ExpRew{\MDPOP{C,\rta,\sk,\hh}}~.
  \end{align*}
\end{theorem}

\begin{proof}
    See \Cref{a:op}.
\end{proof}

\paragraph{Discussion}
infinity if not memory safe, expected ticks if memory safe




